Simplicial volume of manifolds fibering with connected structure group

In this note we investigate the simplicial volume of fiber bundles with connected structure group. We are able to show that if the structure group is either compact or a Lie group, or if the fiber is aspherical that the simplicial volume of the total space agrees with the simplicial volume of the trivial bundle.

==> Theorem/Representatives.tex <==
\begin{theorem}
\label{thm:SphericalRepresentatives}
  Let $\CompactGroup$ denote a compact connected group and
  $\FundamentalGroupShortHand$ some discrete group, for $n \geq 1$, any
  homology class in
  $
    \bigoplus_{i = 1, \ldots n-1}
    \HomologyOfSpaceObject
      {i}
      {\ClassifyingSpace{\CompactGroup}}
      {\Rationals}
    \otimes
    \HomologyOfSpaceObject
      {n-i}
      {\ClassifyingSpace{\FundamentalGroupShortHand}}{\Rationals}
    \subset
    \HomologyOfSpaceObject
      {n}
      {
        \ClassifyingSpace{\CompactGroup}
        \times
        \ClassifyingSpace{\FundamentalGroupShortHand}
      }
      {\Rationals}
  $
  can be represented by a manifold with fundamental group
  $\FundamentalGroupShortHand$ that fibers over a simply-connected sphere.
\end{theorem}
